Self-adaptation of Genetic Operators Through Genetic Programming Techniques

Here we propose an evolutionary algorithm that self modifies its operators at the same time that candidate solutions are evolved. This tackles convergence and lack of diversity issues, leading to better solutions. Operators are represented as trees and are evolved using genetic programming (GP) techniques. The proposed approach is tested with real benchmark functions and an analysis of operator evolution is provided.

==> prevBib <==
\begin{thebibliography}{50}

	\bibitem{mitchellga}
		M. Mitchell. An intoduction to genetic algorithms. MIT Press, 1996.
	\bibitem{gomezhaea}
		J. Gomez. Self Adaptation of Operator Rates in Evolutionary Algorithms. Conference: Genetic and Evolutionary Computation - GECCO 2004.
	\bibitem{kramer}
		O Kramer. Evolutionary self-adaptation: a survey of operators and strategy parameters.
		Evolutionary Intelligence 2010.
	\bibitem{maruo}
	Marcos H. Maruo, Heitor S. Lopes, Myriam R. Delgado. Self-Adapting Evolutionary Parameters: Encoding Aspects for 	Combinatorial Optimization 	Problems. Evolutionary Computation in Combinatorial Optimization: 5th European 	Conference, EvoCOP 2005, Lausanne, Switzerland, March 30 - April 1, 2005.
	\bibitem{younes}
	Abdunnaser Younes, Shawki Areibi, Paul Calamai and Otman Basir (2008). Adapting Genetic Algorithms for Combinatorial Optimization Problems in Dynamic Environments, Advances in Evolutionary Algorithms, Xiong Zhihui (Ed.)
	\bibitem{clrs}
	Introduction to algorithms, Cormen et al, 2001.
	\bibitem{nofreelunch}
	H. Wolpert, G. Macready. No Free Lunch Theorems for Optimization. IEEE TRANSACTIONS ON EVOLUTIONARY COMPUTATION, 	VOL. 1, NO. 1, APRIL 1997.
	\bibitem{cormen}
	TH Cormen. Introduction to algorithms 3rd edition. MIT press.
	\bibitem{garey}
	 M. R. Garey and D. S. Johnson. Computers and Intractability: A Guide to the Theory of NP-	Completeness. W. H. Freeman, New York, 1979	 	 
	\bibitem{hanser}
	Hansen and Ostermeier, Adapting arbitrary normal mutation distributions in evolution strategies: The covariance matrix adaptation. In Proceedings of the 1996 IEEE International Conference on Evolutionary Computation, pp. 312-317.
		\bibitem{schwefel}
	HANS-GEORG BEYER and HANS-PAUL SCHWEFEL, Evolution strategies, A comprehensive introduction. Natural computing, 2002.	
	\bibitem{treedistance}
		KAIZHONG ZHANG AND DENNIS SHASHA, SIMPLE FAST ALGORITHMS FOR THE EDITING DISTANCE BETWEEN TREES AND RELATED PROBLEMS,
	1989 Society for Industrial and Applied Mathematics.
	
	\bibitem{agoston}
	Agoston Endre Eiben, Parameter Control in Evolutionary Algorithms, IEEE TRANSACTIONS ON EVOLUTIONARY COMPUTATION, VOL. 3, NO. 2.

	
\end{thebibliography}
